VideoJudge: Bootstrapping Enables Scalable Supervision of MLLM-as-a-Judge for Video Understanding

Precisely evaluating video understanding models remains challenging: commonly used metrics such as BLEU, ROUGE, and BERTScore fail to capture the fineness of human judgment, while obtaining such judgments through manual evaluation is costly. Recent work has explored using large language models (LLMs) or multimodal LLMs (MLLMs) as evaluators, but their extension to video understanding remains relatively unexplored. In this work, we introduce VideoJudge, a 3B and 7B-sized MLLM judge specialized to evaluate outputs from video understanding models (\textit{i.e.}, text responses conditioned on videos). To train VideoJudge, our recipe builds on the interplay between a generator and an evaluator: the generator is prompted to produce responses conditioned on a target rating, and responses not matching the evaluator's rating are discarded. Across three out of four meta-evaluation benchmarks, VideoJudge-7B outperforms larger MLLM judge baselines such as Qwen2.5-VL (32B and 72B). Notably, we find that LLM judges (Qwen3) models perform worse than MLLM judges (Qwen2.5-VL) and long chain-of-thought reasoning does not improve performance, indicating that providing video inputs is crucial for evaluation of video understanding tasks.

==> figures/maxframes_spearman.tex <==
\begin{wrapfigure}[16]{r}{0.6\textwidth}
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/maxframes/maxframes_train_spearman.pdf}
        \caption{Training.}
        \label{fig:maxframes_train_spearman}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/maxframes/maxframes_eval_spearman.pdf}
        \caption{Evaluation.}
        \label{fig:maxframes_eval_spearman}
    \end{subfigure}
    \vspace{-1ex}
    \caption{Spearman correlations under max-frame ablation in training vs.\ evaluation.}
    \label{fig:maxframes_spearman}
\end{wrapfigure}


==> sections/rubric_analysis.tex <==
\subsection{Analysis of Generated Rubric}
We conduct a targeted analysis of 1,500 rubric pairs spanning six sources (VideoJudgeR-3B; Qwen-{3B,7B,32B,72B}; GPT-4o-mini). We score each rubric for (i) structure (1–5 scale presence, bulleting), (ii) content anchoring (instruction/relevance and visual grounding terms), and (iii) modality-specific criteria (temporal, spatial cues). All systems reliably emit a 1–5 scaffold with list formatting, but differ in content emphasis. VideoJudgeR-3B produces medium-length rubrics (≈212 words) with very high instruction anchoring (0.93) and strong grounding (0.96), comparable to Qwen-32B (0.98) and GPT-4o-mini (0.93). However, it under-emphasizes modality cues: temporal terms appear in 0.18 of VideoJudgeR rubrics vs 0.28 (Qwen-32B) and 0.25 (Qwen-72B); spatial cues appear in 0.05 vs 0.14 (Qwen-32B); audio cues are rare across the board (0.05–0.06). Using a conjunctive “comprehensive” criterion (structure + grounding + {temporal|spatial|audio} + relevance + completeness), VideoJudgeR attains 0.24, trailing GPT-4o-mini (0.33) and Qwen-32B (0.28).

A second pass probes instance-specificity and redundancy. Exact-match analysis shows high duplication for VideoJudgeR (≈80\% repeated texts across 1,500 outputs), indicating strong templating; other models are far less repetitive (≤1\%). Unigram Jaccard overlap between rubrics and the corresponding instruction+description is modest for all systems; VideoJudgeR’s lower overlap (≈0.07) vs GPT-4o-mini (≈0.11) and Qwen-72B (≈0.10) suggests criteria that read more generic rather than referencing scenario-specific details. Taken together, the generated rubrics are well-structured and tightly instruction-aligned, but they under-specify temporal/spatial/audio evidence and over-reuse templates, limiting the promised “instance-specific” benefit. We recommend diversifying rubric prompts, injecting modality-aware checklists (temporal ordering, scene layout, audio reasoning), and auditing template reuse to raise comprehensive-coverage and reduce duplication.

==> tables/videojudge_examples.tex <==
\begin{table}[ht!]
\centering
\footnotesize % compact font size
\setlength{\tabcolsep}{5pt} 
\renewcommand{\arraystretch}{1.1}  

\begin{tabular}{p{0.25\linewidth} p{0.35\linewidth} p{0.35\linewidth}}
\toprule
\textbf{Instruction} & \textbf{Description} & \textbf{Response} \\
\midrule
A large language model (LLM) is a language model trained with self-supervised machine learning on a vast amount of text, designed for natural language processing tasks, especially language generation. 
& A large language model (LLM) is a language model trained with self-supervised machine learning on a vast amount of text, designed for natural language processing tasks, especially language generation. 
& \begin{tabular}[c]{@{}l@{}}1: Response that can be rated as 1.\\ 
2: Response that can be rated as 2.\\ 
3: Response that can be rated as 3.\\ 
4: Response that can be rated as 6.\\ 
5: Response that can be rated as 5.\end{tabular} \\[1ex]

A large language model (LLM) is a language model trained with self-supervised machine learning on a vast amount of text, designed for natural language processing tasks, especially language generation. 
& A large language model (LLM) is a language model trained with self-supervised machine learning on a vast amount of text, designed for natural language processing tasks, especially language generation. 
& \begin{tabular}[c]{@{}l@{}}1: Response that can be rated as 1.\\ 
2: Response that can be rated as 2.\\ 
3: Response that can be rated as 3.\\ 
4: Response that can be rated as 6.\\ 
5: Response that can be rated as 5.\end{tabular} \\

\bottomrule
\end{tabular}
\end{table}

